Optimal Multiserver Scheduling with Unknown Job Sizes in Heavy Traffic

We consider scheduling to minimize mean response time of the M/G/k queue with unknown job sizes. In the single-server case, the optimal policy is the Gittins policy, but it is not known whether Gittins or any other policy is optimal in the multiserver case. Exactly analyzing the M/G/k under any scheduling policy is intractable, and Gittins is a particularly complicated policy that is hard to analyze even in the single-server case. In this work we introduce monotonic Gittins (M-Gittins), a new variation of the Gittins policy, and show that it minimizes mean response time in the heavy-traffic M/G/k for a wide class of finite-variance job size distributions. We also show that the monotonic shortest expected remaining processing time (M-SERPT) policy, which is simpler than M-Gittins, is a 2-approximation for mean response time in the heavy traffic M/G/k under similar conditions. These results constitute the most general optimality results to date for the M/G/k with unknown job sizes. Our techniques build upon work by Grosof et al., who study simple policies, such as SRPT, in the M/G/k; Bansal et al., Kamphorst and Zwart, and Lin et al., who analyze mean response time scaling of simple policies in the heavy-traffic M/G/1; and Aalto et al. and Scully et al., who characterize and analyze the Gittins policy in the M/G/1.

==> figure_macros.tex <==
\input{rank_examples_data}

\makeatletter

% The calc library needs this.
\catcode`\$=3 % math shift

\usetikzlibrary{backgrounds, math, shapes, positioning, decorations.markings}

\def\@above{above}
\def\@below{below}
\def\@negative{-}
\newcommand{\downmode}{%
  \def\@above{below}
  \def\@below{above}
  \def\@negative{}}

\newcommand{\xscale}{12}
\newcommand{\yscale}{6}
\newcommand{\ticksize}{2.5}
\newcommand{\arrowsize}{5}
\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\xscaleload}{%
  \renewcommand{\xscale}{150}
  \renewcommand{\yscale}{10}}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negative(\ticksize)/\yscale})
  node[\@below] {\ifempty{#1}{$#2$}{#1}\vphantom{by}};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})
  node[left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});}
\newcommand{\xguidept}[2]{%
  \ifempty{#1}{}{%
    \draw[axis] \projx{#2} -- \projxheight{#2}{{\@negative(\ticksize)/\yscale}}
    node[\@below] {#1\vphantom{by}}};
  \draw[guide] \projx{#2} -- #2;}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {#3$\vphantom{by}$} -- ({#1 + \xarrowsize}, 0) node[right] {#4$\vphantom{by}$};
  \draw[axis, ->] (0, \@negative\ticksize/\yscale)
  node[\@below] {#5$\vphantom{by}$} -- (0, {#2 + \yarrowsize})
  node[\@above] {#6$\vphantom{by}$};}

\newcommand{\axesxtorsor}[4]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {$0$} -- ({#1 + \xarrowsize}, 0) node[right] {#3};
  \draw[axis, ->] (0, 0) -- (0, {#2 + \yarrowsize})
  node[\@above] {#4};}

\newcommand{\point}[2][primary]{%
  \filldraw[#1, very thick] #2 circle (1.8mu);}

\newcommand{\jump}[4][primary]{%
  \point[#1, fill=white]{(#2, #3)}
  \point[#1]{(#2, #4)}}

\newcommand{\plotlegend}[1][%
  $\Delta \to 0$ limit \\ (lower bound)]{%
  \node[anchor=west, align=left] at (1.13, 32) {%
    $\Delta = 0$ \\ (exact analysis)};
  \draw[primary] (1.1, 25) -- +(0, 14);
  \node[anchor=west, align=left] at (1.13, 62) {#1};
  \draw[bubble] (1.1, 55) -- +(0, 14);}

\newcommand{\snakefirst}[2]{#1 parabola bend #1 \midpt{#1}{#2}}
\newcommand{\snakesecond}[2]{\midpt{#1}{#2} parabola bend #2 #2}
\newcommand{\snake}[2]{\snakefirst{#1}{#2} -- \snakesecond{#1}{#2}}

\newcommand{\intervallabel}[3]{%
  \begin{scope}
    \node (A) at \projx{#1} {};
    \node (B) at \projx{#2} {};
    \node[\@above=1.5pt, inner sep=0pt] at \midpt{(A)}{(B)} {%
      \footnotesize #3\vphantom{ly}};
  \end{scope}}
\newcommand{\intervalsnake}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- \snake{#3}{#4} -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 \snake{#3}{#4};
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakefirst}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #3 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #3 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakesecond}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #4 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #4 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalspecial}[6][--]{%
  \begin{scope}[on background layer]
    \fill[#2]
      \projx{#3}
      -- #3
      parabola bend #4 #4
      parabola bend #4 #5
      -- \projx{#5};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3;
  \intervallabel{#3}{#5}{#6}}
\newcommand{\discarded}[2]{%
  \interval{discarded}{#1}{#2}{}}
\newcommand{\original}[2]{%
  \interval{original}{#1}{#2}{$0$-old}}
\newcommand{\recycled}[3][]{%
  \interval{recycled}{#2}{#3}{\ifempty{#1}{}{$#1$-}old}}

\newcommand{\Isnake}{%
  \draw[primary, name path=rank]
  \snake{(0, 3)}{(1.5, 7)}
  -- \snake{(1.5, 7)}{(2, 4)}
  -- \snake{(2, 4)}{(3.25, 12)}
  -- \snake{(3.25, 12)}{(5.25, 6)}
  -- \snake{(5.25, 6)}{(5.75, 5)}
  -- \snake{(5.75, 5)}{(8.25, 9)}
  -- \snake{(8.25, 9)}{(10.5, 3)}
  -- \snake{(10.5, 3)}{(12.5, 9)};
  \draw[primary, dotted] \snakefirst{(12.5, 9)}{(14.9, 7)};}

\tikzset{%
  figure/.style={x=\xscale, y=\yscale, thick, font=\small,
    baseline={([yshift={-\ht\strutbox}]current bounding box.north)}},
  axis/.style={thick},
  guide/.style={black!30, densely dashed},
  primary/.style={very thick, color=green!67!black},
  secondary/.style={ultra thick, densely dotted, color=purple!95!black}}

\catcode`\$=13 % active
\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m-gittins-k"
%%% End:

